Quantization effects and convergence properties of rigid formation control systems with quantized distance measurements

In this paper, we discuss quantization effects in rigid formation control systems when target formations are described by inter-agent distances. Because of practical sensing and measurement constraints, we consider in this paper distance measurements in their quantized forms. We show that under gradient-based formation control, in the case of uniform quantization, the distance errors converge locally to a bounded set whose size depends on the quantization error, while in the case of logarithmic quantization, all distance errors converge locally to zero. A special quantizer involving the signum function is then considered with which all agents can only measure coarse distances in terms of binary information. In this case, the formation converges locally to a target formation within a finite time. Lastly, we discuss the effect of asymmetric uniform quantization on rigid formation control.

==> Makefile <==
all: IJRNC_Quantization.pdf

clean:
	$(RM) *~ *.pdf *.dvi *.log *.aux *.bbl *.blg *.toc *.lol *.loa *.lox \
		*.lot *.out *.lg *.tmp *.xref *.lof .*.swp

IJRNC_Quantization.pdf: IJRNC_Quantization.tex
	pdflatex IJRNC_Quantization
	bibtex IJRNC_Quantization
	pdflatex IJRNC_Quantization
	pdflatex IJRNC_Quantization


==> cosa.tex <==
\begin{tikzpicture}
	[
  use Hobby shortcut,
  vec1/.style={
    decorate,
    decoration={
      markings,      % v-- can fine-tune arrow position and rotation
      mark=at position 0.1 with {\arrow[rotate=5]{stealth}},
    }
  },
  vec2/.style={
    decorate,
    decoration={
      markings,      % v-- here again---fine-tune as needed
      mark=at position 0.080 with {\arrow{stealth}},
      mark=at position 0.206 with {\arrow{stealth reversed}},
      mark=at position 0.800 with {\arrow{stealth reversed}},
      mark=at position 0.930 with {\arrow{stealth}},
    }
  },
]
\draw circle (1);
\draw (0,0) ellipse (3 and 1.5);
\draw (0,0) ellipse (4 and 2.5);
\draw (0,0) ellipse (5 and 3.5);

	\node at (0,0) {$F_{approx}$};
	\node at (0,-1.7) {$V(e) = a_1$};
	\node at (0,-2.7) {$V(e) = a_2$};
	\node at (0,-3.7) {$V(e) = a_3$};
	\node at (1,1.8) {$\tilde{\mathcal{L}} V(e) <0$};
	\draw[-stealth, line width=1.4] (4.5,2) .. (3,1.5) .. (0.4,1.3) .. (0,1);
\end{tikzpicture}

